LNMap: Departures from Isomorphic Assumption in Bilingual Lexicon Induction Through Non-Linear Mapping in Latent Space

Most of the successful and predominant methods for bilingual lexicon induction (BLI) are mapping-based, where a linear mapping function is learned with the assumption that the word embedding spaces of different languages exhibit similar geometric structures (i.e., approximately isomorphic). However, several recent studies have criticized this simplified assumption showing that it does not hold in general even for closely related languages. In this work, we propose a novel semi-supervised method to learn cross-lingual word embeddings for BLI. Our model is independent of the isomorphic assumption and uses nonlinear mapping in the latent space of two independently trained auto-encoders. Through extensive experiments on fifteen (15) different language pairs (in both directions) comprising resource-rich and low-resource languages from two different datasets, we demonstrate that our method outperforms existing models by a good margin. Ablation studies show the importance of different model components and the necessity of non-linear mapping.

==> backup-results-old_style.tex <==

We present our results on low-resource and resource-rich languages from MUSE dataset in Tables \ref{tab:low-resource-results} and \ref{tab:high-resource-results}, respectively, and the results on VecMap dataset in Table \ref{tab:dinu-results}. We present the results in \textit{precision@1}, which means how many times one of the correct translations of a source word is predicted as the top choice. For each of the cases, we show results on seed dictionary of three different sizes including 1-to-1 and 1-to-many mappings;  \textbf{``1K Unique''} and \textbf{``5K Unique''} contain 1-to-1 mappings of 1000 and 5000 source-target pairs respectively, while \textbf{``5K All''} contains 1-to-many mappings of all 5000 source and target words, that is, for each source word there can be multiple target words. Through experiments and analysis, our goal is to assess the following questions. 
\begin{enumerate}[label=(\roman{*}),topsep=0pt]
    \item Does \lnmap\ improve over the best existing methods in terms of mapping accuracy on low-resource languages (\cref{subsec:low-resource-con})? \vspace{-0.5em}
    \item How well does \lnmap\ perform on resource-rich languages (\cref{subsec:high-resource-con-dinu})?
    \vspace{-0.5em}
    \item Which components of \lnmap\ attribute to improvements (\cref{subsec:dissection})?
\end{enumerate}


%\Ni Does \lnmap\ improve over the best existing methods in terms of mapping accuracy on low-resource languages? (Section \ref{subsec:low-resource-con})? \Nii How well does \lnmap\ perform on resource-rich languages? (Section \ref{subsec:high-resource-con-dinu})? \Niii Which components of \lnmap\ attribute to improvements (Section \ref{subsec:dissection})?


%\begin{enumerate}[label=(\roman*)]
%\vspace{-0.5em}
%\setlength\itemsep{-0.3em}
%    \item Does \lnmap\ improve over the best existing methods in terms of mapping accuracy on low-resource languages? (Section \ref{subsec:low-resource-con})? 
%    \item How well does \lnmap\ perform on resource-rich languages? (Section \ref{subsec:high-resource-con-dinu})?
%    \item Which components of \lnmap\ attribute to improvements (Section \ref{subsec:dissection})?
% \end{enumerate}
 


\subsection{Performance on Low-resource Languages} \label{subsec:low-resource-con}
%\vspace{-0.2em}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Conneau low resource

\begingroup
\setlength{\tabcolsep}{3pt}
\begin{table*}[t!]
\centering
%\small
\footnotesize
\scalebox{0.76}{\begin{tabular}{l|cc|cc|cc|cc|cc|cc|cc|cc|cc|cc||c}
%\toprule

&\multicolumn{2}{c}{\textbf{En-Ms}} & \multicolumn{2}{c}{\textbf{En-Fi}} &    \multicolumn{2}{c}{\textbf{En-Et}} & \multicolumn{2}{c}{\textbf{En-Tr}} & \multicolumn{2}{c}{\textbf{En-El}} & \multicolumn{2}{c}{\textbf{En-Fa}} & \multicolumn{2}{c}{\textbf{En-He}} & \multicolumn{2}{c}{\textbf{En-Ta}} & \multicolumn{2}{c}{\textbf{En-Bn}} & \multicolumn{2}{c}{\textbf{En-Hi}} &
\textbf{\blue{Avg.}}
\\

& \textbf{$\rightarrow$} & \textbf{$\leftarrow$} & 
  \textbf{$\rightarrow$} & \textbf{$\leftarrow$} & 
  \textbf{$\rightarrow$} & \textbf{$\leftarrow$} &
  \textbf{$\rightarrow$} & \textbf{$\leftarrow$} & 
  \textbf{$\rightarrow$} & \textbf{$\leftarrow$} & 
  \textbf{$\rightarrow$} & \textbf{$\leftarrow$} &
  \textbf{$\rightarrow$} & \textbf{$\leftarrow$} & 
  \textbf{$\rightarrow$} & \textbf{$\leftarrow$} & 
  \textbf{$\rightarrow$} & \textbf{$\leftarrow$} &
  \textbf{$\rightarrow$} & \textbf{$\leftarrow$} &
\\ 
\midrule
\textbf{GH Distance} & 
\multicolumn{2}{c|}{0.49} & \multicolumn{2}{c|}{0.54} & \multicolumn{2}{c|}{0.68} & \multicolumn{2}{c|}{0.41} & \multicolumn{2}{c|}{0.46} & \multicolumn{2}{c|}{0.39} & \multicolumn{2}{c|}{0.45} & \multicolumn{2}{c|}{0.29} & \multicolumn{2}{c|}{0.49} & 
\multicolumn{2}{c||}{0.56}  &        
\\ 
\midrule
\multicolumn{11}{l}{\textbf{Unsupervised Baselines}}  \\

\newcite{Artetxe-2018-acl} & 49.0 & 49.7 & 49.8 & 63.5 & 33.7 & 51.2 & 52.7 & 63.5 & 47.6 & 63.4 & 33.4 & 40.7 & 43.8 & 57.5 & 0.0 & 0.0 & 18.4 & 23.9 & 39.7 & 48.0 & \blue{41.5} \\

\newcite{conneau2018word} &  46.2 & 0.0 & 38.4 & 0.0 & 19.4 & 0.0 & 46.4 & 0.0 & 39.5 & 0.0 & 30.5 & 0.0 & 36.8 & 53.1 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & \blue{15.5} \\

\newcite{mohi-joty:2019}  & \blue{54.1} & \blue{51.7} &  \blue{44.8} &  \blue{62.5} & \blue{31.8} & \blue{48.8} & \blue{51.3} & \blue{61.7} & \blue{47.9} & \blue{63.5} & \blue{36.7} & \blue{44.5} & \blue{44.0} & \blue{57.1} & \blue{0.0} & \blue{0.0} & \blue{0.0} & \blue{0.0} & \blue{0.0} & \blue{0.0} & \blue{35.0}\\

\midrule
\multicolumn{20}{c}{{\small{{Supervision With \hl{\textbf{``1K Unique''}} Seed Dictionary}}}} \\
\midrule

% \multicolumn{11}{l}{\textbf{Supervised\blue{/Semi-supervised} Baselines}}  \\
\multicolumn{11}{l}{\textbf{Sup.\blue{/Semi-sup.} Baselines}}  \\

\newcite{artetxe2017acl} & 36.5 & 41.0 & 40.8 & 56.0 & 21.3 & 39.0 & 39.5 & 56.5 & 34.5 & 56.2 & 24.1 & 35.7 & 30.2 & 51.7 & 5.4 & 12.7 & 6.2 & 19.9 & 22.6 & 38.8 & \blue{33.5}\\

\newcite{artetxe2018aaai} & 35.3 & 34.0 & 30.8 & 40.8 & 21.6 & 32.6 & 33.7 & 43.3 & 32.0 & 46.4 & 22.8 & 27.6 & 32.27 & 39.1 & 7.3 & 11.9 & 11.3 & 15.7 & 26.2 & 30.7  & \blue{28.8}\\

\newcite{conneau2018word} & 46.2 & 44.7 & 46.0 & 58.4 & 29.3 & 40.0 & 44.8 & 58.5 & 42.1 & 56.5 & 31.6 & 38.4 & 38.3 & 52.4 & 11.7 & 16.0 & 14.3 & 19.7 & 32.5 & 42.3  & \blue{38.2}\\

 \newcite{joulin-2018} & 31.4 & 30.7 & 30.4 & 41.4 & 20.1 & 26.0 & 30.7 & 36.5 & 28.8 & 43.6 & 18.7 & 23.1 & 33.5 & 34.3 & 6.0 & 10.1 & 7.6 & 11.3 & 20.7 & 25.7  & \blue{25.6}\\

\newcite{jawanpuria2018learning} & \blue{40.0} & \blue{39.6} & \blue{37.5} & \blue{50.7} & \blue{24.9} & \blue{38.4} & \blue{39.7} & \blue{49.7} & \blue{36.6} & \blue{52.9} & \blue{26.1} & \blue{33.0} & \blue{35.1} & \blue{44.5} & \blue{10.0} & \blue{15.9} & \blue{12.0} & \blue{19.7} & \blue{30.5} & \blue{37.1}  & \blue{33.7}  \\

\newcite{patra-19}  & \blue{40.4} & \blue{41.4} & \blue{44.3} & \blue{59.8} & \blue{21.0} & \blue{40.4} & \blue{41.4} & \blue{58.8} & \blue{37.1} & \blue{58.9} & \blue{26.5} & \blue{39.6} & \blue{38.4} & \blue{54.1} & \blue{6.4} & \blue{15.1} & \blue{6.1} & \blue{18.1} & \blue{24.9} & \blue{35.4}   & \blue{35.5}\\
 
\sc{\textbf{LNMap}}  & \textbf{50.1} & \textbf{50.6} & \textbf{54.3} & \textbf{64.3} & \textbf{39.1} & \textbf{51.1} & \textbf{52.9} & \textbf{64.0} & \textbf{48.3} & \textbf{62.1} & \textbf{35.3} & \textbf{41.3} & \textbf{45.3} & \textbf{54.9} & \textbf{18.3} & \textbf{24.3} & \textbf{19.7} & \textbf{30.3} & \textbf{36.9} & \textbf{49.3}   & \blue{\textbf{44.6}}

\\
\midrule
\multicolumn{20}{c}{{\small{Supervision With \hl{\textbf{``5K Unique''}} Seed Dictionary}}} \\
\midrule

%\multicolumn{11}{l}{\textbf{Supervised\blue{/Semi-supervised} Baselines}}  \\
\multicolumn{11}{l}{\textbf{Sup.\blue{/Semi-sup.} Baselines}}  \\

\newcite{artetxe2017acl} &36.5 & 42.0 & 40.8 & 57.0 & 22.4 & 39.6 & 39.6 & 56.7 & 37.2 & 56.4 & 26.0 & 35.3 & 31.6 & 51.9 & 6.2 & 13.4 & 8.2 & 21.3 & 23.2 & 38.3   & \blue{34.2} \\

\newcite{artetxe2018aaai} & 54.6 & 52.5 & 48.8 & 65.2 & 38.2 & 54.8 & 52.0 & 65.1 & 47.5 & 64.6 & 38.4 & 42.4 & 47.4 & 57.4 & 18.4 & 25.79 & 21.9 & 31.8 & 40.3 & 49.5  & \blue{45.8}\\

\newcite{conneau2018word} & 46.4 & 45.7 & 46.0 & 59.2 & 31.0 & 41.7 & 45.9 & 60.1 & 43.1 & 56.8 & 31.6 & 37.7 & 38.4 & 53.4 & 14.3 & 19.1 & 15.0 & 22.6 & 32.9 & 42.8  & \blue{39.2}\\

\newcite{joulin-2018} & 50.0 & 49.3 & 53.0 & 66.1 & 39.8 & 52.0 & \textbf{54.0} & 61.7 & 47.6 & 63.4 & \textbf{39.6} & 42.2 & \textbf{53.0} & 56.3 & 16.0 & 24.25 & 21.3 & 27.0 & 38.3 & 47.5  & \blue{45.2}\\

\newcite{jawanpuria2018learning} & \textbf{\blue{51.0}} & \blue{49.8} & \blue{47.4} & \blue{65.1} & \blue{36.0} & \blue{49.8} & \blue{49.3} & \blue{63.9} & \blue{46.6} & \blue{62.3} & \blue{36.6} & \blue{40.8} & \blue{44.1} & \blue{56.1} & \blue{16.1} & \blue{23.2} & \blue{18.6} & \blue{25.9} & \blue{37.5} & \blue{45.9}   & \blue{43.3} \\

\newcite{patra-19}   & \blue{46.0} & \blue{46.7} & \blue{48.6} & \blue{60.9} & \blue{33.1} & \blue{47.2} & \blue{48.3} & \blue{61.0} & \blue{44.2} & \blue{60..9} & \blue{34.4} & \blue{40.7} & \blue{43.5} & \blue{56.5} & \blue{15.3} & \blue{22.0} & \blue{15.2} & \blue{25.0} & \blue{34.7} & \blue{43.5}   & \blue{41.4}\\
 
\sc{\textbf{LNMap}}  & {50.2} & \textbf{54.6} & \textbf{54.7} & \textbf{69.2} & \textbf{41.8} & \textbf{57.2} & 52.0 & \textbf{66.6} & \textbf{49.7} & \textbf{65.5} & 36.8 & \textbf{44.5} & 47.3 & \textbf{58.7} & \textbf{20.7} & \textbf{30.7} & \textbf{22.2} & \textbf{36.2} & \textbf{39.1} & \textbf{51.6}   & \blue{\textbf{47.5}}
 
\\
\midrule
\multicolumn{20}{c}{{\small{Supervision With \hl{\textbf{``5K All''}} (``5K Unique'' Source Words) Seed Dictionary}}} \\
\midrule

% \multicolumn{11}{l}{\textbf{Supervised Baselines}}  \\
\multicolumn{11}{l}{\textbf{Sup.\blue{/Semi-sup.} Baselines}}  \\

\newcite{artetxe2017acl} & 37.0 & 41.6 & 40.8 & 57.0 & 22.7 & 39.5 & 38.8 & 56.9 & 37.5 & 57.2 & 25.4 & 36.3 & 32.2 & 52.1 & 5.9 & 14.1 & 7.7 & 21.7 & 22.4 & 38.3  & \blue{34.3}\\

\newcite{artetxe2018aaai} & 55.2 & 51.7 & 48.9 & 64.6 & 37.4 & 54.0 & 52.2 & 63.7 & 48.2 & 65.0 & 39.0 & 42.6 & 47.6 & 58.0 & 19.6 & 25.2 & 21.1 & 30.6 & \textbf{40.4} & 50.0   & \blue{45.8}\\

\newcite{conneau2018word} & 46.3 & 44.8 & 46.4 & 59.0 & 30.9 & 42.0 & 45.8 & 59.0 & 44.4 & 57.4 & 31.8 & 38.8 & 39.0 & 53.4 & 15.1 & 18.4 & 15.5 & 22.4 & 32.9 & 44.4  & \blue{39.4}\\

\newcite{joulin-2018} & \textbf{51.4} & 49.1 & \textbf{55.6} & 65.8 & 40.0 & 50.2 & \textbf{53.8} & 61.7 & \textbf{49.1} & 62.8 & \textbf{40.5} & 42.4 & \textbf{52.2} & 57.9 & 17.7 & 24.0 & 20.2 & 26.9 & 38.2 & 47.1  & \blue{45.3}\\

\newcite{jawanpuria2018learning}  & \textbf{\blue{51.4}} & \blue{47.7} & \blue{46.7} & \blue{63.4} & \blue{33.7} & \blue{48.7} & \blue{48.6} & \blue{61.9} & \blue{46.3} & \blue{61.8} & \blue{38.0} & \blue{40.9} & \blue{43.1} & \blue{56.7} & \blue{16.5} & \blue{23.1} & \blue{19.3} & \blue{25.6} & \blue{37.7} & \blue{44.1}   & \blue{42.8}\\

\newcite{patra-19}   & \blue{48.4} & \blue{43.8} & \blue{53.2} & \blue{63.8} & \blue{36.3} & \blue{48.3} & \blue{51.8} & \blue{59.6} & \blue{48.2} & \blue{61.8} & \blue{38.4} & \blue{39.3} & \blue{51.6} & \blue{55.2} & \blue{16.5} & \blue{22.7} & \blue{17.5} & \blue{26.7} & \blue{36.2} & \blue{45.4}   & \blue{43.3}\\
 
\sc{\textbf{LNMap}}  & 50.4 & \textbf{56.0} & 55.1 & \textbf{71.5} & \textbf{41.9} & \textbf{57.5} & 52.6 & \textbf{66.3} & \textbf{49.1} & \textbf{67.1} & 36.5 & \textbf{43.7} & 47.4 & \textbf{61.0} & \textbf{19.9} & \textbf{32.0} & \textbf{22.5} & \textbf{36.6} & 38.7 & \textbf{52.7}   & \blue{\textbf{47.9}}

\\
\bottomrule
\end{tabular}}
\vspace{-0.5em}
\caption{Translation accuracy (P@1) on \textbf{low-resource} languages on \textbf{MUSE dataset} using {fastText} embeddings. } 
\label{tab:low-resource-results} 
\end{table*}
\endgroup



Most of the unsupervised models fail in the majority of the low-resource languages \cite{vulic-19-emnlp}. On the other hand, the performance of supervised models on low-resource languages was not satisfactory, \blue{especially with small seed dictionary.} Hence, we first compare \lnmap 's performance on the these languages. {From Table \ref{tab:low-resource-results},  we see that on average \lnmap\ outperforms every baseline by a good margin \red{(1.9\% - 6.4\% from the best baseline)}.}

%In Table \ref{tab:low-resource-results},  we see \red{very impressive performance} of \lnmap\ for \textbf{``1K Unique''} seed dictionary. 
For {``1K Unique''} seed dictionary, \lnmap\ exhibits impressive performance. In all the 20 translation tasks, it outperforms all the (semi-)supervised baselines by a wide margin. If we compare with \citet{joulin-2018}, a state-of-the-art supervised model, \lnmap's average improvement is $\sim$$19\%$, which is remarkable. Compared to other baselines, the average margin of improvement is also quite high -- $11.1\%, 15.8\%, 6.4\%, 10.9\%,$ and $9.2\%$ improvements over \citet{artetxe2017acl}, \newcite{artetxe2018aaai}, \newcite{conneau2018word}, \newcite{jawanpuria2018learning}, and \newcite{patra-19}, respectively. We see that among the supervised baselines, \citet{conneau2018word}'s model performs better than others.

% it achieves the highest accuracy with a large margin compared to the baselines. 
% \blue{    on  \textbf{``1K Unique''} dictionary.}

If we increase the dictionary size, we can still see the dominance of \lnmap\ over the baselines. For {{``5K Unique''}} seed dictionary, it performs better than the baselines on {16/20 translation tasks}, while for {``5K All''} seed dictionary, the best performance by \lnmap\ is on {13/20 translation tasks.} 

One interesting thing to observe is that, under resource constrained setup \lnmap's performance is {impressive}, making it suitable for very low-resource languages like En-Ta, En-Bn, and En-Hi. 

%other baseline models' performance improve a lot compared to  . This means \lnmap\ can perform impressively even under a limited sized seed dictionary.

Now if we look at the performance of unsupervised baselines on low-resource languages, we see that \citet{conneau2018word}'s model fails to converge on the majority of the translation tasks (12/20), {while the model of \citet{mohi-joty:2019} fails to converge on En$\leftrightarrow$Ta, En$\leftrightarrow$Bn, and En$\leftrightarrow$Hi.} Although the most robust unsupervised method of \citet{Artetxe-2018-acl} performs better than the other unsupervised approaches, it still fails to converge on En$\leftrightarrow$Ta tasks. If we compare its performance with \lnmap, we see that our model outperforms the best unsupervised model of \citet{Artetxe-2018-acl} on 18/20 low-resource translation tasks.



%##########################


\subsection{Results on Resource-rich Languages} \label{subsec:high-resource-con-dinu}
%\vspace{-0.2em}

In this section, we discuss  \lnmap's performance on resource-rich languages from both datasets - MUSE and VecMap. Table \ref{tab:high-resource-results} shows the results for 5 resource-rich language pairs (10 translation tasks) from MUSE. We see that \lnmap\ in its default setting achieves the highest accuracy in {6, 2, and 2 translation tasks} for  {``1K Unique''}, {``5K Unique''}, and {``5K All''} seed dictionaries, respectively. 


%In the VecMap dataset, there are 6 translations tasks for resource-rich languages. Here \lnmap\ performs better than other baselines on {1, 0, and 0 translation tasks} for  \textbf{``1K Unique''},  \textbf{``5K Unique''}, and \textbf{``5K All''} seed dictionaries, respectively. 

The results on the VecMap dataset are shown in Table \ref{tab:dinu-results}, where there are 3 resource-rich language pairs (En-Es, En-It, En-De), and one low-resource pair (En-Fi). Here, \lnmap\ (in its default setting) performs better than the best baselines only on 1/8 translation task for {``1K Unique''} seed, and for the other seeds, it  does not show any improvements. 

%For the other two seed dictionaries, \lnmap\ 

\begingroup
\setlength{\tabcolsep}{3pt}
\begin{table}[t!]
\centering
\footnotesize
\scalebox{0.6}{\begin{tabular}{l|cc|cc|cc|cc|cc||c}
%\toprule
&\multicolumn{2}{c}{\textbf{En-Es}}  &        \multicolumn{2}{c}{\textbf{En-De}} &\multicolumn{2}{c}{\textbf{En-It}}& \multicolumn{2}{c}{\textbf{En-Ar}} &\multicolumn{2}{c}{\textbf{En-Ru}}&
\textbf{\blue{Avg.}}
\\
& \textbf{$\rightarrow$} & \textbf{$\leftarrow$} & \textbf{$\rightarrow$} & \textbf{$\leftarrow$} & 
\textbf{$\rightarrow$} & \textbf{$\leftarrow$} & 
\textbf{$\rightarrow$} & \textbf{$\leftarrow$} & 
\textbf{$\rightarrow$} & \textbf{$\leftarrow$} 
\\   
\midrule
\textbf{GH Distance} & \multicolumn{2}{c|}{0.21} & \multicolumn{2}{c|}{0.31} & \multicolumn{2}{c|}{0.19} & \multicolumn{2}{c|}{0.46} & \multicolumn{2}{c}{0.46} &

\\
\midrule

\multicolumn{6}{l}{\textbf{Unsupervised Baselines}} & \\

\newcite{Artetxe-2018-acl} & 82.2 & 84.4 & 74.9 & 74.1 & 78.9 & 79.5 & 33.2 & 52.8 & 48.93 & 65.0 & 67.4 \\

\newcite{conneau2018word} & 81.8 & 83.7 & 74.2 & 72.6 & 78.3 & 78.1 & 29.3 & 47.6 & 41.9 & 59.0 & 64.7  \\

\newcite{mohi-joty:2019} & \blue{82.7} & \blue{84.7} & \blue{75.4} & \blue{74.3} & \blue{79.0} & \blue{79.6} & \blue{36.3} & \blue{52.6} & \blue{46.9} & \blue{64.7} & 67.6 \\
  

\midrule
\multicolumn{10}{c}{{\small{Supervision With \hl{\textbf{``1K Unique''}} Seed Dictionary}}} \\
\midrule

% \multicolumn{6}{l}{\textbf{Supervised Baselines}}  & \\
\multicolumn{6}{l}{\textbf{Sup.\blue{/Semi-sup.} Baselines}}  \\

\newcite{artetxe2017acl} &  81.0 & {83.6} & 73.8 & 72.4 & 76.6 & {77.8} & 24.9 & 44.9 & 46.3 & 61.7 & 64.3 \\

\newcite{artetxe2018aaai} & 73.8 & 76.6 & 62.5 & 57.6 & 67.9 & 70.0 & 25.8 & 37.3 & 40.2 & 49.5 & 56.2\\

\newcite{conneau2018word} & {81.2} & 82.8 & 73.6 & 73.0 & {77.6} & 76.6 & 34.7 & 46.4 & 48.5 & 60.6 & 65.5\\

\newcite{joulin-2018} & 70.8 & 74.1 & 59.0 & 54.0 & 62.7 & 67.2 & 22.4 & 32.2 & 39.6 & 45.4 & 52.8\\
 
\newcite{jawanpuria2018learning}  & \blue{75.1} & \blue{77.3} & \blue{66.0} & \blue{62.6} & \blue{69.3} & \blue{71.6} & \blue{28.4} & \blue{40.6} & \blue{41.7} & \blue{53.9}  & 58.6\\
 
\newcite{patra-19}  & {\blue{81.9}} & {\blue{83.8}} & \blue{74.6} & {{73.1}} & \textbf{{\blue{78.0}}} & {\blue{78.1}} & \blue{29.8} & \blue{50.9} & \blue{46.3} & {63.6} & 66.0\\ 
 
\sc{\textbf{LNMap}}  & 80.7 & 81.7 & {74.7} & {73.1} & 76.7 & 76.1 & \textbf{40.3} & \textbf{54.1} & \textbf{51.3} & {63.7} & 67.2\\

\sc{\textbf{LNMap}}\ \textbf{(Lin. AE)} & \textbf{82.1} & \textbf{85.4} & \textbf{75.3} & \textbf{74.9} & 77.5 & \textbf{79.6} & 35.6 & 53.7 & 50.8 & \textbf{67.01} & \textbf{68.2}

\\
\midrule
\multicolumn{10}{c}{{\small{Supervision With \hl{\textbf{``5K Unique''}} Seed Dictionary}}} \\
\midrule

% \multicolumn{6}{l}{\textbf{Supervised Baselines}}  & \\
\multicolumn{6}{l}{\textbf{Sup.\blue{/Semi-sup.} Baselines}}  \\

\newcite{artetxe2017acl} & 81.3 & 83.3 & 72.8 & 72.6 & 76.3 & 77.6 & 24.1 & 45.3 & 47.5 & 60.3 & 64.1\\

\newcite{artetxe2018aaai} & 80.8 & 84.5 & 73.3 & 74.3 & 77.4 & 79.7 & 42.0 & 54.7 & 51.5 & {68.2} & 68.7\\

\newcite{conneau2018word} & 81.6 & 83.5 & 74.1 & 72.7 & 77.8 & 77.2 & 34.3 & 48.5 & 49.0 & 60.7 &  66.0\\

\newcite{joulin-2018} & \textbf{83.4} & {85.4} & \textbf{77.0} & \textbf{76.4} & \textbf{78.7} & \textbf{81.6} & 41.3 & 54.0 & \textbf{58.1} & 67.4 & \textbf{70.4}\\
 
\newcite{jawanpuria2018learning} & \blue{81.3} & {\blue{86.3}} & \blue{74.5} & \blue{75.9} & \blue{78.6} & \blue{81.3} & \blue{38.7} & \blue{53.4} & \blue{52.3} & \blue{67.6} & 68.9\\
 
\newcite{patra-19}  & \blue{82.2} & \blue{84.6} & \blue{75.6} & \blue{73.7} & \blue{77.8} & \blue{78.6} & \blue{35.0} & \blue{51.9} & \blue{52.2} & \blue{65.2} & 69.5\\ 
 

\sc{\textbf{LNMap}}  & 80.7 & 82.3 & 74.9 & 73.6 & 77.5 & 78.1 & \textbf{42.4} & \textbf{56.8} & 54.5 & 67.6 & 68.9\\

\sc{\textbf{LNMap}}\ \textbf{(Lin. AE)} & 82.5 & \textbf{86.5} & 75.5 & 75.4 & 78.2 & 81.1 & 39.1 & 56.7 & 56.0 & \textbf{68.8} & 70.0
 
\\
\midrule
\multicolumn{10}{c}{{\small{Supervision With \hl{\textbf{``5K All''}}(5K Unique Source Words) Seed Dictionary}}} \\
\midrule

% \multicolumn{6}{l}{\textbf{Supervised Baselines}}  & \\
\multicolumn{6}{l}{\textbf{Sup.\blue{/Semi-sup.} Baselines}}  \\

\newcite{artetxe2017acl} & 81.2 & 83.5 & 72.8 & 72.5 & 76.0 & 77.5 & 24.4 & 45.3 & 47.3 & 61.2 & 64.2\\

\newcite{artetxe2018aaai} & 80.5 & 83.8 & 73.5 & 73.5 & 77.1 & 79.2 & 41.2 & 55.5 & 50.5 & 67.3  & 68.2\\

\newcite{conneau2018word} & 81.6 & 83.2 & 73.7 & 72.6 & 77.3 & 77.0 & 34.1 & 49.4 & 49.8 & 60.7 & 66.0\\

\newcite{joulin-2018} & \textbf{84.4} & \textbf{86.4} & \textbf{79.0} & {76.0} & {79.0} & {81.4} & \textbf{42.2} & 55.5 & \textbf{57.4} & 67.0  & \textbf{70.9}\\
 
\newcite{jawanpuria2018learning} & \blue{81.4} & \blue{85.5} & \blue{74.7} & \textbf{\blue{76.7}} & \blue{77.8} & \blue{80.9} & \blue{38.1} & \blue{53.3} & \blue{51.1} & \blue{67.6}  & 68.7\\
 
\newcite{patra-19}  & \blue{84.0} & \textbf{\blue{86.4}} & \blue{78.7} & \blue{76.4} & \textbf{\blue{79.3}} & \textbf{\blue{82.4}} & \blue{41.1} & \blue{53.9} & \blue{57.2} & \blue{64.8} & 70.4\\ 
 

\sc{\textbf{LNMap}}  & 80.5 & 83.7 & 73.6 & 75.0 & 76.9 & 78.7 & 41.7 & \textbf{59.6} & 54.9 & \textbf{69.3} & 69.4\\

\sc{\textbf{LNMap}}\ \textbf{(Lin. AE)} & 82.6 & \textbf{86.4} & 74.8 & 75.5 & 77.8 & 80.8 & 39..1 & 57.0 & 54.6 & 68.5 & 69.7

\\
\bottomrule
\end{tabular}}
\vspace{-0.5em}
\caption{Word translation accuracy (P@1) on \textbf{resource-rich} languages on \textbf{MUSE dataset} using {fastText}} %embeddings (trained on {Wikipedia}).} 
\label{tab:high-resource-results} 
\end{table}
\endgroup



In general, we see that \lnmap's performance is not quite satisfactory on resource-rich languages compared to low-resource languages. To investigate the reason, we first measure the geometric similarity of the language pairs for the translation tasks using the \textbf{Gromov-Hausdorff (GH)} distance \cite{patra-19}, which is recently proposed to quantitatively estimate isometry between two embedding spaces.\footnote{\href{https://github.com/joelmoniz/BLISS}{https://github.com/joelmoniz/BLISS}} %For calculating \textbf{GH Distance}, we consider 5K most frequent words of the two languages.
From the measurements (Tables \ref{tab:low-resource-results}-\ref{tab:high-resource-results}), we see that etymologically {close language pairs} have lower {GH distance} compared to etymologically distant and low-resource language pairs. 


%We then conduct another set of experiments for the resource-rich languages on both datasets. In the experiment, we replace \lnmap's non-linear \emph{autoencoder} with a linear one {(the mappers are still non-linear)}. Table \ref{tab:lin-autoenc-results} shows the results of our experiment for resource-rich languages on both datasets. We see that for \textbf{``1K Unique''} dictionary \lnmap\ achieves the highest accuracies on 10 out of 12 translation tasks (compare Table \ref{tab:lin-autoenc-results} with Table \ref{tab:high-resource-results} and \ref{tab:dinu-results}). For the other two dictionary results,  we also see improvements -- \lnmap\ achieves highest accuracies in 7 out of 12 tasks for \textbf{``5K Unique''} and  5 out of 12 tasks for \textbf{``5K All''}.
We then conduct another set of experiments for the resource-rich languages on both datasets. In the experiment, we replace \lnmap's non-linear \emph{autoencoder} with a linear one (note that the mappers are still non-linear). We refer this variant of \lnmap\ as ``{\sc{\textbf{LNMap}}\ \textbf{(Lin. AE)}}'' in Tables \ref{tab:high-resource-results}-\ref{tab:dinu-results}. From the results, we see that for {``1K Unique''} dictionary our method achieves the highest accuracy on 13/16 translation tasks in the two datasets. For the other two seed dictionaries, we also see improvements -- for {{``5K Unique''}} seed dictionary, our method performs better than the baselines on {10/16 translation tasks}, while for {``5K All''}, we achieve the best performance on {8/16 translation tasks.} 




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Dinu Dataset results}

\begingroup
\begin{table}[t!]
\centering
\small
\setlength{\tabcolsep}{4pt}
\scalebox{0.65}{\begin{tabular}{l|cc|cc|cc|cc||c}
%\toprule
&\multicolumn{2}{c}{\textbf{En-Es}}  &        \multicolumn{2}{c}{\textbf{En-It}} &\multicolumn{2}{c}{\textbf{En-De}}& \multicolumn{2}{c}{\textbf{En-Fi}} &
\textbf{\blue{Avg.}}
\\
&\textbf{$\rightarrow$} & \textbf{$\leftarrow$} & \textbf{$\rightarrow$} & \textbf{$\leftarrow$} & 
\textbf{$\rightarrow$} & \textbf{$\leftarrow$} & 
\textbf{$\rightarrow$} & \textbf{$\leftarrow$} 
\\       
\midrule

\multicolumn{9}{l}{\textbf{Unsupervised Baselines}} \\

\newcite{Artetxe-2018-acl} & 36.9 & 31.6 & 47.9 & 42.3 & 48.3 & 44.1 & 32.9 & 33.5 & 39.7\\

\newcite{conneau2018word} & 34.7 & 0.0 & 44.9 & 38.7 & 0.0 & 0.0 & 0.0 & 0.0 & 14.8\\

\newcite{mohi-joty:2019} & \blue{37.4} & \blue{31.9} & \blue{47.6} & \blue{42.5} & \blue{0.0} & \blue{0.0} & \blue{0.0} & \blue{0.0}  & 19.9\\

\midrule
\multicolumn{10}{c}{{\small{Supervision With \hl{\textbf{``1K Unique''}} Seed Dictionary}}} \\
\midrule

%\multicolumn{9}{l}{\textbf{Supervised Baselines}}\\
\multicolumn{9}{l}{\textbf{Sup.\blue{/Semi-sup.} Baselines}}  \\

\newcite{artetxe2017acl}  & 33.3 & 27.7 & 43.9 & 38.1 & 46.8 & 40.8 & 30.4 & 26.0 & 35.9\\

\newcite{artetxe2018aaai} &  29.0 & 20.0 & 38.6 & 29.2 & 36.3 & 26.0 & 25.8 & 15.0 & 27.5\\

\newcite{conneau2018word} & \textbf{35.7} & {30.8} & {45.4} & 38.3 & {46.9} & {42.3} & {29.1} & 27.2 & 37.0\\

\newcite{joulin-2018} & 24.2 & 17.9 & 33.9 & 25.1 & 31.6 & 25.5 & 21.9 & 14.5 & 24.4\\
 
\newcite{jawanpuria2018learning}  & \blue{31.5} & \blue{23.2} & \blue{39.2} & \blue{32.4} & \blue{39.1} & \blue{30.9} & \blue{26.8} & \blue{21.4} & 30.6\\ 

\newcite{patra-19}   & \blue{31.4} & \blue{30.5} & \blue{30.9} & \blue{38.8} & \textbf{\blue{47.9}} & {\blue{43.7}} & \textbf{\blue{30.5}} & {\blue{31.6}} & 35.7\\

 
\sc{\textbf{LNMap}}  & 33.5 & 30.4 & 45.3 & {40.1} & 43.3 & 42.0 & 25.9 & {30.3} & 36.4
\\

\sc{\textbf{LNMap}}\ \textbf{(Lin. AE)} & 34.6 & \textbf{33.2} & \textbf{46.4} &	\textbf{41.1} & 45.3 & \textbf{44.5} & 27.5 & \textbf{35.6} & \textbf{37.6}
 

\\
\midrule
\multicolumn{10}{c}{{\small{Supervision With \hl{\textbf{``5K Unique''}} Seed Dictionary}}} \\
\midrule

%\multicolumn{9}{l}{\textbf{Supervised Baselines}} \\
\multicolumn{9}{l}{\textbf{Sup.\blue{/Semi-sup.} Baselines}}  \\

\newcite{artetxe2017acl} & 33.3 & 27.6 & 43.9 & 38.4 & 46.0 & 41.1 & 30.9 & 25.7 & 35.9\\

\newcite{artetxe2018aaai} & \textbf{37.6} & {34.0} & 45.7 & {41.6} & {47.2} & {45.0} & {34.0} & {38.8} & 40.5\\

\newcite{conneau2018word} & 36.0 & 31.1 & 46.0 & 38.8 & 47.6 & 43.2 & 31.1 & 28.2 & 37.8\\

\newcite{joulin-2018} & 34.2 & 31.1 & 43.1 & 37.2 & 44.5 & 41.9 & 30.9 & 34.7 & 37.2\\
 
\newcite{jawanpuria2018learning}   & \blue{36.9} & \blue{33.3} & {\blue{47.1}} & \blue{39.9} & {\blue{47.7}} & \blue{44.6} & \textbf{\blue{35.1}} & \blue{38.0} & 40.3\\ 

\newcite{patra-19}   & \blue{34.3} & \blue{31.6} & \blue{41.1} & \blue{39.3} & \blue{47.5} & \blue{43.6} & \blue{30.7} & \blue{33.4} & 37.7\\

\sc{\textbf{LNMap}}  & 35.7 & 31.0 & {46.3} & 40.5 & 45.1 & 43.5 & 31.2 & 35.9 & 38.7\\

\sc{\textbf{LNMap}}\ \textbf{(Lin. AE)} & \textbf{37.6} & \textbf{34.6} & \textbf{47.6} &	\textbf{41.8} & \textbf{47.9} & \textbf{46.5} & 33.4 & \textbf{40.2 } & \textbf{41.2}
 
\\
\midrule
\multicolumn{10}{c}{{\small{Supervision With \hl{\textbf{``5K All''}} (5K Unique Source Words) Seed Dictionary}}} \\
\midrule

%\multicolumn{9}{l}{\textbf{Supervised Baselines}} \\
\multicolumn{9}{l}{\textbf{Sup.\blue{/Semi-sup.} Baselines}}  \\

\newcite{artetxe2017acl} & 32.7 & 28.1 & 43.8 & 38.0 & 47.4 & 40.8 & 30.8 & 26.2 & 36.0\\

\newcite{artetxe2018aaai} & {38.2} & {33.4} & {47.3} & {41.6} & {47.2} & {44.8} & \textbf{34.9} & {38.6} & 40.8\\

\newcite{conneau2018word} & 36.1 & 31.2 & 45.7 & 38.5 & 47.2 & 42.8 & 31.2 & 28.3 & 37.7\\

\newcite{joulin-2018} & 35.5 & 31.2 & 44.6 & 37.6 & 46.6 & 41.7 & 32.1 & 34.4 & 38.0\\

\newcite{jawanpuria2018learning} & \blue{37.5} & \blue{33.1} & \textbf{\blue{47.6}} & \blue{40.1} & \textbf{\blue{48.8}} & {\blue{45.1}} & \blue{34.6} & \blue{37.7} & 40.6\\ 

\newcite{patra-19}   & \blue{34.5} & \blue{32.1} & \blue{46.2} & \blue{39.5} & \blue{48.1} & \blue{44.1} & \blue{31.0} & \blue{33.6} & 39.4\\
 
\sc{\textbf{LNMap}}  & 35.7 & 31.6 & 46.0 & 40.1 & 45.4 & 43.6 & 29.8 & 37.3 & 38.7\\

\sc{\textbf{LNMap}}\ \textbf{(Lin. AE)} & \textbf{38.7} & \textbf{34.7} &	\textbf{47.6} &	\textbf{42.1} &	46.9 &	\textbf{45.6} & 33.1 & \textbf{39.5} & \textbf{41.0}

\\
\bottomrule
\end{tabular}}
\vspace{-0.5em}
\caption{Word translation accuracy (P@1) on \textbf{VecMap dataset} using {CBOW} embeddings.} 
\label{tab:dinu-results} 
\end{table}
\endgroup



We also evaluate {\sc{{LNMap}}\ {(Lin. AE)}} on low-resource tasks \red{(Table \ref{tab:low-resource-results})}. We observe that for low-resource language pairs, the performance of the linear autoencoder framework is worse than the non-linear one. \textit{GH distance} measures corroborate this observation. Low-resource language pairs' high \textit{GH distance} measure implies that English and those languages embedding spaces are far from isomorphism. {Hence, we need strong non-linearity for those distant languages.}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%linear autoencoder results for high-resource languages
\begin{comment}
\begingroup
\setlength{\tabcolsep}{3pt}
\begin{table}[t!]
\centering
\footnotesize
\scalebox{0.80}{\begin{tabular}{cc|cc|cc||cc|cc|cc}
%\toprule
\multicolumn{6}{c||}{\textbf{MUSE} Dataset}  &        \multicolumn{6}{c}{\textbf{VecMap} Dataset} \\
\midrule

\multicolumn{2}{c}{\textbf{En-Es}}  &        \multicolumn{2}{c}{\textbf{En-It}}&
\multicolumn{2}{c||}{\textbf{En-De}}& 
\multicolumn{2}{c}{\textbf{En-Es}} &        \multicolumn{2}{c}{\textbf{En-It}}&
\multicolumn{2}{c}{\textbf{En-De}}
\\
\textbf{$\rightarrow$} & \textbf{$\leftarrow$} & \textbf{$\rightarrow$} & \textbf{$\leftarrow$} & 
\textbf{$\rightarrow$} & \textbf{$\leftarrow$} & 
\textbf{$\rightarrow$} & \textbf{$\leftarrow$} & 
\textbf{$\rightarrow$} & \textbf{$\leftarrow$} & 
\textbf{$\rightarrow$} & \textbf{$\leftarrow$} 
\\       
\midrule

\multicolumn{12}{c}{{\small{Supervision With \hl{\textbf{``1K Unique''}} Seed Dictionary}}} \\
\midrule

\textbf{82.1} & \textbf{85.4} & {77.6} & \textbf{79.6} & \textbf{75.3} & \textbf{74.9} & 34.6 & \textbf{33.2} & \textbf{46.4} &	\textbf{41.1} & 45.3 & \textbf{44.5}\\


\midrule
\multicolumn{12}{c}{{\small{Supervision With \hl{\textbf{``5K Unique''}} Seed Dictionary}}} \\
\midrule
82.5 &	\textbf{86.5} & 78.2 & 81.1 & 75.5 & 75.4 & \textbf{37.6} & \textbf{34.6} & \textbf{47.6} &	\textbf{41.8} & \textbf{47.9} & \textbf{46.5}\\


\midrule
\multicolumn{12}{c}{{\small{Supervision With \hl{\textbf{``5K All''}} (5K Unique Source Words) Seed Dictionary}}} \\
\midrule
82.6 & \textbf{86.4} & 77.8 & 80.8 & 74.8 & 75.5 & \textbf{38.7} & \textbf{34.7} &	\textbf{47.6} &	42.1 &	46.87 &	\textbf{45.6}
\\
\bottomrule
\end{tabular}}
\vspace{-0.5em}
\caption{Word translation accuracy (P@1) on \textbf{resource-rich} languages for both \textbf{MUSE} and \textbf{VecMap} dataset using \textbf{linear autoencoder} in \lnmap.} 
\label{tab:lin-autoenc-results} 
\end{table}
\endgroup

\end{comment}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%










%\vspace{-0.2em}
\subsection{Dissecting \lnmap\ }
\label{subsec:dissection}
%\vspace{-0.3em}
\input{ablation.tex}
%\vspace{-0.8em}


